Identification and Estimation of Dynamic Games with Unknown Information Structure

We develop an empirical framework for analyzing dynamic games when the underlying information structure is unknown to the analyst. We introduce \textit{Markov correlated equilibrium}, a dynamic analog of Bayes correlated equilibrium, and show that its predictions coincide with the Markov perfect equilibrium predictions attainable when players observe richer signals than the analyst assumes. We provide tractable methods for informationally robust estimation, inference, and counterfactual analysis. We illustrate the framework with a dynamic entry game between Starbucks and Dunkin' in the US and study the role of informational assumptions.

==> S.1.Introduction/S.1.2.Notation.tex <==
% Notation
\begin{notation}
Throughout the paper, we will use the following notation. $\mathbb{P}(\cdot)$ and $\mathbb{E}(\cdot)$ are generic notations for mathematical probability and expectations. If $Y$ is a random variable whose support is a finite set $\mathcal{Y}$, we let $p\left(y\right)\equiv p_{y}\equiv\mathbb{P}\left(Y=y\right)$ for $y\in\mathcal{Y}$. Similarly, $p\left(y\vert x\right)\equiv p_{y\vert x}\equiv \mathbb{P} \left(Y=y\vert X=x\right)$ denotes the conditional probability of $Y=y$ given $X=x$. We let $\Delta_{y}\equiv\Delta\left(\mathcal{Y}\right)$ denote the probability simplex on $\mathcal{Y}: p\in\Delta_{y}$ if and only if $p_{y}\geq0$ for all $y\in\mathcal{Y}$ and $\sum_{y\in\mathcal{Y}}p_{y}=1$. Similarly, we let $p\in\Delta_{y\vert x}$ if and only if $p_{y\vert x}\geq0$ for each $y\in\mathcal{Y}$ and $\sum_{y\in\mathcal{Y}}p_{y\vert x}=1$. We also use the convention that writes an action profile as $a=\left(a_{1},...,a_{I}\right)=\left(a_{i},a_{-i}\right)$. For an arbitrary set $S$, $\vert S\vert$ represents the number of elements of the set. 
\end{notation}
